FSD50K: An Open Dataset of Human-Labeled Sound Events

Most existing datasets for sound event recognition (SER) are relatively small and/or domain-specific, with the exception of AudioSet, based on over 2M tracks from YouTube videos and encompassing over 500 sound classes. However, AudioSet is not an open dataset as its official release consists of pre-computed audio features. Downloading the original audio tracks can be problematic due to YouTube videos gradually disappearing and usage rights issues. To provide an alternative benchmark dataset and thus foster SER research, we introduce FSD50K, an open dataset containing over 51k audio clips totalling over 100h of audio manually labeled using 200 classes drawn from the AudioSet Ontology. The audio clips are licensed under Creative Commons licenses, making the dataset freely distributable (including waveforms). We provide a detailed description of the FSD50K creation process, tailored to the particularities of Freesound data, including challenges encountered and solutions adopted. We include a comprehensive dataset characterization along with discussion of limitations and key factors to allow its audio-informed usage. Finally, we conduct sound event classification experiments to provide baseline systems as well as insight on the main factors to consider when splitting Freesound audio data for SER. Our goal is to develop a dataset to be widely adopted by the community as a new open benchmark for SER research.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> S2_Related.tex <==

This Section discusses the most important datasets for SER (i.e., SET and SED).
The selection criteria is based on the number of Google Scholar citations, as well as popularity and/or size for the most recent ones. 

\subsection{Datasets for Sound Event Tagging or Classification}
Table \ref{tab:dataset_sota} summarizes some aspects of a few most relevant datasets. 
For comparison, the proposed FSD50K is listed at the bottom.
%of a smaller selection of the few most relevant datasets, in our view, after discarding synthetic datasets. 
\textit{m-c} and \textit{m-l} in the \textit{task} column correspond to multi-class and multi-label.
The basic common aspect in SET datasets is that labels are provided at the clip-level (without timestamps), usually regarded as \textit{weak} labels.

\begin{table*}[ht]
%\vspace{-1mm}
\caption{A selection of most relevant datasets for SET.}
%\vspace{+3mm}
\centering
\begin{tabular}{l|ccccccc}
\toprule
\textbf{dataset}             & \textbf{clips} & \textbf{clip length} & \textbf{duration}  & \textbf{classes} & \textbf{task} & \textbf{source} & \textbf{domain/task}\\
\midrule
UrbanSound8k \cite{salamon2014dataset} (2014)  & 8732         & $\leq$4s        &8.8h        &10 bal    & m-c   & Freesound  & urban sounds \\
ESC-50 \cite{piczak2015esc} (2015)            &2000           &5s               &2.8h        &50 bal    & m-c  & Freesound   \\ 
CHiME-home \cite{foster2015chime} (2015)      & 6138          & 4s              &6.8h        &7 unbal   & m-l   & CHiME    & domestic sounds\\ 
%TUT Sound events 2016 \cite{Mesaros2016_EUSIPCO} & 32   & 3-5min    & $\approx$2h   &18 unbal   & m-l SED   & TUT  \\
%TUT Sound events 2017 \cite{DCASE2017challenge}  & 32   & 3-5min    & $\approx$2h   &6 unbal   & m-l SED   & TUT  \\
AudioSet (2017)  \cite{gemmeke2017audio}     & $\approx$2.1M   &$\approx$10s    &$\approx$5731h &527 (un)bal  & m-l  & YouTube  \\ 
%SINS (2018)  \cite{Dekkers2017}               & xxx        & 10s            & xxx          &9   & XXXXX      & SED, m-c, unbalanced domestic sounds \\
FSDnoisy18k \cite{Fonseca2019learning} (2019) & 18,532    & 0.3-30s         & 43h         & 20 unbal    & m-c   & Freesound  & noisy labels\\ 
FSDKaggle2019 \cite{Fonseca2019audio} (2019)   & 29,266   & 0.3-30s         & 103h          & 80 unbal & m-l   & Freesound/YFCC & noisy labels \& domain mismatch\\ 
SONYC-UST v2.2 \cite{cartwright2019sonyc} (2020) & 18,515     & 10s              & 51h          & 31 unbal & m-l   & SONYC & urban sounds\\ 
\textbf{FSD50K} (2020)                         & 51,197     & 0.3-30s         & 108h         & 200 unbal & m-l   & Freesound \\ 

%\midrule
\bottomrule
\end{tabular}
\label{tab:dataset_sota}
%\vspace{-2mm}
\end{table*}

%-----------Before the release of AudioSet, the most widely used datasets were XYZ,
\subsubsection{Datasets Released Before AudioSet}
Before the release of AudioSet, the most widely used datasets for SET have been UrbanSound8k \cite{salamon2014dataset}, ESC-50 \cite{piczak2015esc}, and to a lesser extent CHiME-home \cite{foster2015chime}.
All of them feature short audio chunks and a total duration of less than 10h. 
Curiously, the two former are one of the few multi-class balanced datasets in SER---most datasets are unbalanced and/or multi-label---and also the most widely used (besides AudioSet).
Remarkable in terms of data per class are UrbanSound8k and CHiME-home, counting with a significant amount of clips per-class; nonetheless, part of this abundance comes from the fact that many clips are actually slices coming from the same original recording.
ESC-50 features an unprecedented large vocabulary at the time, however it suffers from data scarcity (only 40 clips/class).
Common to all mentioned datasets, is that they provide a k-fold cross validation setup---a practice that tended to disappear after the AudioSet release.

%\subsubsection{AudioSet and AudioSet Ontology}
\subsubsection{AudioSet}
Google's AudioSet is the largest dataset of sound events ever released, consisting of $\approx$2.1M audio clips manually labeled using 527 classes of the AudioSet Ontology \cite{gemmeke2017audio}.
AudioSet is the first dataset to put emphasis on general-purpose SER, enabling sound event recognizers to describe a huge variety of sound classes, thus aiming at the transcription of most everyday sounds.
AudioSet is split into a train and an evaluation set, and it is highly imbalanced, with some classes being particularly common (e.g. \textit{Music} and \textit{Speech}) while others are much more scarce (e.g. \textit{Toothbrush}).
Yet, the public release provides a balanced train partition of 22,176 clips in addition to the full unbalanced train set.
While the dataset is manually labeled in full (which entails a tremendous endeavour), its unprecedented size and coverage inevitably comes at the expense of a less precise labeling.
In particular, labeling error in AudioSet is estimated at above 50\% for $\approx$18\% of the classes.\footnote{See \url{https://research.google.com/audioset/dataset/index.html} for details on how the quality is estimated, accessed 25th June 2020.\label{foot_aset_noise}}
As mentioned in Sec. \ref{sec:intro}, the official release provides audio features instead of audio waveforms.
The AudioSet Ontology (a subset of which is used to organize FSD50K) is described in Sec. \ref{ssec:acqui}.


\subsubsection{Datasets Released After AudioSet}
After AudioSet, some of the released datasets for SET are task-dependent, designed to enable the study of particular SER problems. 
Examples include FSDnoisy18k \cite{Fonseca2019learning} or FSDKaggle2019 \cite{Fonseca2019audio}, focused on learning in conditions of noisy labels and/or acoustic mismatch.
Other datasets are domain-specific, with a vocabulary focused on a specific scope, such as SONYC-UST for urban sounds \cite{cartwright2019sonyc}.
Compared to pre-AudioSet datasets, these are slightly larger, especially in terms of duration as they feature longer clips (sometimes of variable length), but also in terms of vocabulary.
In addition, they are unbalanced, and the default data split transitioned to a development/evaluation (or train/test) separation.
Beyond those listed in Table \ref{tab:dataset_sota}, another large dataset is BirdVox-14SD for bird sounds.
%Beyond those listed in Table \ref{tab:dataset_sota}, another large dataset is BirdVox-14SD, totalling over 14k clips of avian flight calls with 18 species annotation \cite{cramer2020chirping}.
Last, a recent large-vocabulary dataset with a substantial amount of data is VGGSound \cite{chen2020vggsound}, an audio-visual dataset consisting of $\approx$200k video clips from Youtube encompassing 300 classes.
It presents, however, several shortcomings for SER.
The focus is put on audio-visual correspondence due to which the dataset is created mostly through automatic computer vision techniques---hence some classes have a clear visual connotation, e.g., \textit{people eating noodle}.
Also, while the dataset is singly-labeled (one machine-generated label per clip), the authors recognize that clips can contain a mixture of sounds.
Upon inspection of the vocabulary, it seems likely that sound events from different classes co-occur in the same clip (of 10s length), thus creating missing labels---for example, \textit{cat growling} and \textit{cat meowing}, or a combination of \textit{sea waves}, \textit{sailing}, or \textit{wind noise}.
%, or \textit{ocean burbling}.
Missing labels is a form of label noise found to impact sound recognizers \cite{fonseca2020addressing}. 
While measures can be taken to mitigate their effect on training, in evaluation they can lead to misleading results---an issue that we specifically address in FSD50K (Sec. \ref{ssec:task_gen}).
In addition, VGGSound suffers from the intrinsic problems of being backed by YouTube (Sec. \ref{sec:intro}).

To our knowledge, all datasets listed in Table \ref{tab:dataset_sota} are labelled manually (except a portion of FSDnoisy18k and FSDKaggle2019 which is purposefully included for the study of noisy labels).
All listed dataset releases are freely available, including waveforms, except AudioSet.


\subsection{Datasets for Sound Event Detection}
Early stage datasets for SED were rather small as they were curated through manual annotation of sound events using start and end times (usually regarded as \textit{strong} labels)---this process is especially laborious and sometimes ambiguous.
Examples include TUT Sound events 2016 \cite{Mesaros2016_EUSIPCO} and TUT Sound events 2017 \cite{DCASE2017challenge}, each totalling $\approx$2h of annotated audio.
To overcome this limitation, synthetic datasets became popular for SED, where soundscapes are generated by mixing a set of target sound events taken from other datasets with additional acoustic material.
The main advantage of this approach is the larger control of many dataset aspects---in particular, sound event start/end times are reliable as they are determined by dataset construction.
Further, provided the generation scripts are available, this paradigm allows for increasing dataset size arbitrarily.
%creating different dataset versions to study specific aspects of sound events \cite{serizel2020sound}, or simply 
The main downside of this approach is that the synthesized soundscapes may not always be representative of real-world recordings, as pointed out by \cite{salamon2017scaper}.
This depends on factors such as the user-defined specifications for the generation, or the fact the generated soundscapes are based on combinations of a limited amount of sound event instances.

An early example of this approach is TUT Rare Sound Events 2017 \cite{DCASE2017challenge}.
URBAN-SED \cite{salamon2017scaper} is a dataset synthesized by mixing sound events from the 10 classes of UrbanSound8K with Brownian noise using the Scaper library.
An increasingly popular dataset is DESED \cite{turpault2019sound}, covering 10 classes of domestic sounds.
This dataset is composed of a set of recorded soundscapes from AudioSet (including unlabeled, weakly labeled, and strongly labeled portions), and a synthetic set constructed by mixing sound events from Freesound with additional material.
Other instances of this approach include TAU Spatial Sound Events 2019 \cite{Adavanne2019_DCASE}, for sound event detection and localization, and VOICe \cite{gharib2019voice}, for the study of domain adaptation in SED.
All SED datasets mentioned are unbalanced, pose a multi-label problem, and feature less than a dozen classes (except TUT Sound events 2016, with 18).
% finally SINS
%Another relevant dataset, though not strictly of sound events, is the SINS dataset \cite{Dekkers2017}, consisting of daily activities recorded in a home environment.
%The dataset features a substantial amount of data (almost 150k segments) covering 9 daily activities (e.g., cooking or watching TV) posing a multi-class classification problem.


%\subsection{Datasets for Environmental Sound Recognition}

%============================================================================================
%\subsection{AudioSet and AudioSet Ontology}


%bit of nomenclature

%nodes instead of taxa
%ancestors
%leaves

%============================================================================================
%\subsection{Dataset Creation}

%============================================================================================
%\subsection{Active Learning for Sound Event Recognition}
%Active learnning aims at optimizing a model’s performance with a limited labelling budget REF, typically when a lot of unlabeled data are available, but annotation can be provided only to a limited amount of them.

%Usually AL is based on an iterative process that involves humans in the loop.

%1-selection of samples, commonly based on an estimate of the sample informativeness, thus its usefulness to improve a model. Methods include for example:
%-uncertainty sampling, using the uncertainty of a pre-trained model to classify the sample REF
%-cluster-based sampling, where the centroids of clusters are selected for annotation.
%-disagreement between predictions by different systema (eg pre-trained models and/or similarity measures)

%2Once the estimated relevant samples are selected, they are labeled by humans

%3The newly annotated data can usually have two goals: 
%-use the newly annotated data to propagate their labels to similar samples...
%-Use the updated train set to train a model, which is often used as one of the mechanisms to determine a new batch of samples to annotate, thus closing the iteration loop.

%Additionally, in some cases, a portion of the non-selected unlabeled samples in every iteration is automatically labelled and included in the model training, eg, via propagation of human provided labels to similar examples or with a classic semi-supervised learning approach, using the most confident model predictions to machine-label samples.
%semi-supervised learning, 


==> S3_Creation.tex <==

\subsection{Design Criteria}
\label{ssec:design}
%(0.5)
% this belongs to \subsection{Overall procedure} but it is here for latex drama
\begin{figure*}[ht]
%\begin{figure}[ht]
    %\vspace{-4mm}
    \centering
  \centerline{\includegraphics[width=1.02\textwidth]{IEEEtran/figs/overall_creation_h.pdf}}
    \caption{Overall process of the creation of FSD50K. The process starts from Freesound and the AudioSet Ontology. Stages in green involve automatic data mining, stages in orange correspond to manual annotation tasks, and stages in blue involve data processing to shape the dataset.}
    \label{fig:overall}
    %\vspace{-4mm}
\end{figure*}
% font size mas peque, y cajas tb / fix logos / mirar como quedan los colores en IEEE SPL
As design criteria, we set three basic goals and another three specific goals.
The basic goals are:
\textit{i)} the dataset must be open and fully distributable, \textit{ii)} it must contain a large vocabulary of everyday sounds, and \textit{iii)} it must be expandable in terms of data and vocabulary.
To fulfil these basic goals, we turn to Freesound as a source of data, and to the AudioSet ontology as a vocabulary to organize these data.
Not only these resources feature a large amount of data and classes, respectively, but Freesound is constantly growing through user uploads, and the ontology was designed to be expandable, allowing dataset expansions. 
They are described in Sec. \ref{ssec:acqui}.

In addition, we set three specific goals related to labeling of the dataset and emphasis on the evaluation set.

\subsubsection{Weak Labels}
We opt to label the dataset with weak labels.
%, that is, clip-level labels expressing the presence of a sound event, without temporal location.
The main motivation is that gathering weak labels is simpler, less time consuming and less ambiguous than determining events’ onset/offset (i.e., strong labels).
Weakly supervised learning has demonstrated effectiveness to learn sound event recognizers, both for classification and detection \cite{mcfee2018adaptive}. 
Nonetheless, using weak labels imply certain limitations on training and evaluation, which we highlight in Sec. \ref{ssec:discussion}.

\subsubsection{Label Quality and Dataset Size}
The SER field has witnessed a transition away from small and exhaustively labeled datasets (e.g., \cite{piczak2015esc,salamon2014dataset,foster2015chime}), in favour of larger datasets that inevitably include less precise labelling, such as AudioSet \cite{gemmeke2017audio}.
This occurs mainly because it is intractable to exhaustively annotate large amounts of sound event data.
In our case, we want to seek a trade-off by prioritizing label quality while ensuring a certain amount of data, thus aiming at a medium-size dataset with high label reliability. 
Yet, label noise problems also appear in FSD50K, as in any sound event dataset of certain size (see Sec. \ref{ssec:limit}).

\subsubsection{Emphasis on Evaluation Set}
This is perhaps the design criteria that mostly determines the creation of FSD50K.
%One design criteria that especially drives the creation of FSD50K is to put emphasis on the evaluation set.
Essentially, an evaluation set defines the target behavior in a recognition task, which makes it possibly the most critical part of a dataset.
Consequently, having a comprehensive, diverse, reliably annotated, and real-world representative evaluation set is the key to meaningful systems’ benchmarking.
%CV
The importance of reliable evaluation sets is highlighted by recent research in computer vision which focuses on improving the evaluation and/or validation sets of widely-used datasets---\cite{barz2020we} for CIFAR-10/-100 \cite{krizhevsky2009learning}; and \cite{recht2019imagenet,beyer2020we} for ImageNet \cite{deng2009imagenet}.
%several training alternatives  - but carefully labeled eval sets are still needed.
In addition, alternative learning paradigms to the traditional supervised learning using reliably-labelled datasets start to be promising nowadays.
Specifically, significant progress is being made in the development of sound event recognizers with noisy supervision \cite{fonseca2020addressing} or self-supervision \cite{jansen2018unsupervised}.
These alternatives can minimize the gravity of labelling inaccuracies in the development set, or the need for a labeled development set at all.
However, a carefully curated evaluation set is still critical for benchmarking.
%, regardless of the type of training supervision.
Relatedly, abundant data resources for training are already available, either from AudioSet, or directly from web audio repositories such as Freesound or Flickr (provided appropriate learning strategies are used).
By contrast, to our knowledge, large-vocabulary, carefully-curated evaluation benchmarks are rare---the most prominent being AudioSet’s evaluation set, which suffers from issues of label noise, stability and/or openness (Secs. \ref{sec:intro} and \ref{sec:related}).
By prioritizing the curation of the evaluation set, we contribute to fill this gap.

To tackle the task of labelling the dataset, we consider two options: manual annotation, and incorporating automatic methods in an Active Learning (AL) setting.
% manual
Manual annotation is the conventional approach to dataset labelling, as done in AudioSet \cite{gemmeke2017audio} or ImageNet \cite{deng2009imagenet}.
While this option is very laborious and time consuming, when done properly, we believe it can lead to more reliable results than involving automatic methods in the annotation loop.
%AL
As an alternative, AL aims at maximizing a model’s performance with a limited labelling budget by selecting the most informative data for the model to learn.
%cite Riccardi Hakkani Tur?. 
Usually AL is based on an iterative process involving humans in the loop where automatic methods are used to select the samples to be annotated.
Recent works studying AL for SER (\cite{han2016semi,wang2019active,shuyang2018active,zhao2020active}),
report reduced annotation effort with good performance which, in principle, makes AL appealing for dataset creation.
However, these works focus on recognition tasks with less than a dozen classes, and most of them deal with single-label classification and use pre-labeled datasets, where the human annotation step is simulated by a simple assignment of the existing ground truth.
In addition, it seems the success of these methods is somewhat problem-specific, depending on factors such as the complexity of the classification task or the annotated data available to train automatic methods, as noted in \cite{han2016semi,zhao2020active}.
This casts doubts on the applicability of AL to our more complex scenario, requiring multi-label annotation of samples with a vocabulary of hundreds of classes (some of them rather ambiguous).
%\footnote{In the creation process, we only do this at the last stage, using expert annotators that have undergone extensive training.} 
In this respect, previous work in image recognition evaluates an AL method in two datasets of 10 classes and CIFAR-100 (of 100 classes) \cite{sener2017active}. 
The proposed method is found less effective in CIFAR-100 due to the larger number of classes.
To our knowledge, there is not any released sound event dataset that has used AL strategies in its creation under similar circumstances to ours, and AL in large vocabulary settings has not been studied in SER.
Thus, this is considered a research problem out of the scope of this work.

%decision
Thus, in order to obtain a high-quality labelling, and being aware of the amount of data to annotate and the budget available, we decide to annotate the dataset manually, similarly as done with AudioSet.
While this means a higher human effort, it presents two advantages.
First, manually annotating FSD50K gives us a deeper insight into the data that would not have gained otherwise.
Second, it allows us to have a greater control of the labels gathered, as well as to specify not only the labels but also an estimate of sound predominance (Sec. \ref{ssec:task_val}).
Furthermore, obtaining a set of labels as reliable as possible for this first release is a more favorable starting point for future expansions, which could rely on (semi-) automatic methods to scale up more efficiently at the expense of label noise.

%============================================================================================
\subsection{Overall procedure}
\label{ssec:overall}
%(0.5)
The overall process of the creation of FSD50K is illustrated in Fig. \ref{fig:overall}.
We start from Freesound and the AudioSet Ontology, and we end up with FSD50K.
In every stage, we progressively filter out a quantity of audio clips and classes in the vocabulary.
Each stage is described in the next subsections.


%============================================================================================
\subsection{Data acquisition}
\label{ssec:acqui}
%(0.5)
The starting point for the creation of FSD50K is an abundant source of audio clips, a vocabulary to annotate them, and an infrastructure where they can be loaded and annotation tasks can be carried out. This subsection describes Freesound, the AudioSet Ontology, and the Freesound Annotator, respectively.

%=============
\subsubsection{Freesound}
Freesound\footnote{\url{https://freesound.org/}} is an online collaborative audio clip sharing site that has been supporting diverse research and artistic purposes since 2005 \cite{font2013freesound}.
Freesound has \TODO{XXX} million registered users, over 450,000 audio clips, and more than \TODO{XXX} new clips are added every month.\footnote{Data from July 13th.}
%
The most obvious type of content is audio clips covering a very wide variety of content, from music samples to environmental sounds, including human sounds, audio effects, etc.
Also, users complement the sounds with metadata, e.g., a title, several tags, textual descriptions and comments.
Remarkable are the user-provided tags (at least three per clip), which we leverage in the dataset creation process (Sec. \ref{ssec:nomina}).
Since Freesound is a collaboratively contributed source of data, it is rather heterogeneous in terms of data origin, recording gears, acoustic conditions, or time span of the recordings.
However, quality is prioritized over quantity in terms of audio recording and metadata associated to the files. 
One of the most popular roles of Freesound is the exchange of well-recorded audio samples that are useful for creative purposes such as sound design.
All of the content is released under CC licenses, which conveniently allows distribution.
A number of openly available research datasets containing Freesound audio has been widely used by the community \cite{stowell2013open,salamon2014dataset,piczak2015esc,fonseca2018general,Fonseca2019learning,Fonseca2019audio}, showing its usefulness for the creation of research datasets.

%=============
\subsubsection{AudioSet Ontology}
The AudioSet Ontology\footnote{It can be explored at \url{https://research.google.com/audioset/ontology/index.html}. Sometimes we shall refer to the AudioSet Ontology simply as the ontology.} consists of 632 sound event classes arranged in a hierarchy with a maximum depth of 6 levels \cite{gemmeke2017audio}.
The set of classes covers a very diverse range of everyday sounds, from human and animal sounds, to natural, musical and miscellaneous sounds.
Within these main sound families, the content covered by the ontology includes several axes.
The predominant classes correspond to sound events produced by physical sound sources, but there are also some generated by sound production mechanisms (e.g., deformation or impact of materials that otherwise would radiate no sound).
Then, there is a variety of classes that, strictly, do not correspond to sound events, such as acoustic scenes, categories describing attributes of sound, mathematical signals or abstract classes.
%arrangements of other existing categories, mathematical acoustic signals,
The ontology is provided as a list of 632 python dictionaries,\footnote{\url{https://github.com/audioset/ontology}} each of them including fields such as a Knowledge Graph Machine ID or a textual description, among others.
Note that the AudioSet vocabulary is a subset of 527 classes drawn from the ontology, with the remaining classes being blacklisted or excluded as considered abstract.

% onto for our vocabulary
We use the ontology because it is the most comprehensive set of everyday sounds available, which comes in handy to cover Freesound's heterogeneity.
In addition, the rapid acceptance of AudioSet as a resource for SER research has made the AudioSet Ontology a \textit{de facto} standard for everyday sound organization.
Yet, upon careful inspection of the ontology, we note that improvements could be made in order to make it more consistent as a resource for everyday sound vocabulary, and to make it more suitable for organization of Freesound audio.
However, this task was found to be far from trivial and considered out of the scope of this work.
For FSD50K, we try to focus on a subset of the ontology oriented to the most common physical sources, and less oriented to ambiguous or less represented classes in common everyday situations.

%Similarly, FSD50K is also organized using a subset of the AudioSet Ontology.\footnote{In the following, we shall sometimes refer to the AudioSet Ontology as the ontology.}
We clarify next some ontology-related terms used in the remainder of this paper.
%The 632 classes in the ontology are commonly regarded as \textit{taxa} in the taxonomic nomenclature. 
We shall refer to the 632 classes in the ontology as \textit{nodes} (either \textit{leaf} nodes when they are located at the very bottom of the hierarchy, or \textit{intermediate} nodes otherwise).
We shall also use the ontological terms of \textit{children} and \textit{parents}, as widely used in 
ontology-related genome research \cite{jantzen2011go}.
Note that, by definition, leaf nodes do not have children nodes, while the intermediate nodes do.
Similarly, given a node, we refer to all the parent nodes connecting it to the root of the ontology as \textit{ancestors}.
As an example, let us consider the hierarchical path: \textit{Root} $\rightarrow$ \textit{Natural sounds}  $\rightarrow$ \textit{Thunderstorm} $\rightarrow$ \textit{Thunder}. 
In this path, \textit{Thunder} is a leaf node; \textit{Natural sounds} and \textit{Thunderstorm} are both intermediate nodes; \textit{Thunderstorm} is child of \textit{Natural sounds} and parent of \textit{Thunder}; and \textit{Thunderstorm} and \textit{Natural sounds} are all the ancestors of \textit{Thunder}.


%=============
\subsubsection{Freesound Annotator}
Freesound Annotator\footnote{\url{https://annotator.freesound.org/}} (FSA) is a website that aims at collaboratively creating and curating open audio datasets.
It serves mainly two goals: the management and exploration of datasets, and the creation and verification of annotations.
Currently, it hosts only FSD50K.
Originally released on 2017 as the \textit{Freesound Datasets} platform in our previous work \cite{Fonseca2017freesound}, it has been object of continuous development.
It started by providing basic prototypes for exploring a taxonomy and validating automatically generated annotations.
Additional features were incorporated progressively, including annotation tools and quality control mechanisms (see Secs. \ref{ssec:task_val} and Sec. \ref{ssec:task_gen}).
Monitoring tools allow inspection of a dataset progress as well as debugging capabilities.
FSA uses the Django Python Framework and Postgres as a database.
A database model allows to store, manage and retrieve clips and their annotations.
A user model allows to keep track of users' contributions.
%The platform allows setting pioritization schemes to certain data.
FSA is primarily developed by XF and FF of the authors, and its code is openly available.\footnote{\url{https://github.com/MTG/freesound-datasets/}}

%these models allows for instance to assign some priority score to annotation in order to prioritize certain types of sound and to reach agreement faster on the validation of annotations by several people.
%We also store and keep all the contributions made by any user so that they can be reused in other ways.

%These tools were used by users in order to start gathering annotation and collect feedback for improving the platform.
%Additional features were added for instance for providing clearer guidelines, better category and taxonomy visualisations, and useful answers to typical doubts users were facing.
%Since one of our intention was to open the annotation tools to the public to faster the creation of datasets in a crowdsourcing way, we also implemented some quality control mechanisms for instance by adding test cases in the contribution forms or relying on users' answers redundancy and agreement.
% add a sentence about more examples of additional implemented features
%Additionally, we also concentrated in specialized tools that were used by expert people in order to curate the dataset. % reformulate here, be clearer

%============================================================================================
\subsection{Candidate Labels Nomination}
\label{ssec:nomina}
%(0.5)
We started building FSD50K by automatically populating the classes of the ontology with a number of candidate audio clips from Freesound.
Candidate clips were selected by matching user-provided tags in Freesound to a set of keywords associated with every class.
% based on a process of tag matching leveraging the user-provided tags of Freesound.
The goal is to automatically compile a list of candidate labels per clip, indicating potential presence of sound events.
The process consisted of two steps.

First, we compile a list of keywords for each class.
These are terms related to the class label that are likely to be provided by Freesound users as tags when describing audio clips.
Suitable keywords were found by considering class names and descriptions provided in the ontology, and obtaining most frequent Freesound tags that co-occur with each target class label.
%We also added the Freesound tags after iteratively inspecting Freesound search results obtained when introducing specific query terms related to each class.
After compiling a first version of keywords for all classes, we identified a few classes with very low precision due to pathological inclusion of false positives (e.g., in the \textit{Turkey} class many clips were recordings made in the Eurasian country, instead of containing recordings of the large bird).
To minimize this issue, a refinement process was performed by blacklisting some tags.
%Therefore, the keywords typically include the class label together with additional similar terms used by the Freesound community.
As an example, the keywords defined for the \textit{Meow} class are: “meow”, “meowing”,            "mew", "miaow", and "miaou", as these are the main tags used in Freesound to describe the sound event. 

Second, each class was automatically populated with suitable Freesound clips.
We use the compiled lists of keywords as a mapping between clips in Freesound and class labels in the ontology.
Thus, for each clip, all user-provided tags are examined and, when a tag matches a keyword, the clip becomes a candidate clip for the dataset, and the corresponding class label is nominated as a candidate label for the clip.
We employ the Porter Stemming algorithm for term normalisation to make our matching process more robust \cite{porter1980algorithm}.

%numbers
After this initial process, we were able to map more than 300,000 Freesound clips to the AudioSet classes. 
Because clips in Freesound can widely vary in length, we decided to filter out clips longer than 90s to avoid very large audio clips (this length limit will be further reduced later on).
This left us with a total of 268,261 clips with an average of 2.62 candidate labels.
%discussion
We are aware this label nomination system has flaws as it depends on factors such as class ambiguity and especially the choices of Freesound users when providing tags.
However, it has the advantage of allowing us to easily and rapidly retrieve content for a large variety of classes without training any classifiers.

%out
The outcome of this stage is a list of automatically-generated candidate labels per clip, indicating the potential presence of sound events.
%The pool of candidate labels will be human-validated in the next stage.


%============================================================================================
\subsection{Validation Task}
\label{ssec:task_val}
%(1)
The goal of this stage is to manually validate the candidate labels nominated in the previous stage.
%The input to this stage is

\subsubsection{Initial Prototype of the Annotation Tool}
To this end, we designed and implemented an annotation tool that was deployed in FSA.
Essentially, human raters are presented with a number of audio clips and, for each clip, they must assess the presence of a given sound class. For each class, the annotation process consists of two phases:
\begin{enumerate}
    \item a \textbf{training phase} where raters get familiar with the class by looking at its location in the hierarchy and reading the Audioset-provided textual description. In addition, representative sound examples are provided for inspection.
    \item a \textbf{validation phase}, in which raters are presented with a series of audio clips from that class (up to 72 clips in 6 pages of 12 clips) and prompted the question: \textit{Is $<$class$>$ present in the following sounds?}. In this initial prototype, raters must select among ``Present", ``Not Present", and ``Unsure", similarly as done in \cite{gemmeke2017audio}.
\end{enumerate}

Along with the playable audio and its waveform, raters were also given links to each clip' Freesound page, where the original tags and descriptions can be inspected to aid the validation process.
%Ordering of clips was randomized in order to avoid possible bias effects due to presentation order.

\subsubsection{Internal Quality Assessment (IQA)}
We used the initial prototype to run an Internal Quality Assessment (IQA).
The objective is two-fold: \textit{i) }assess the quality of the candidates produced by the nomination system, and \textit{ii)} collect feedback about the prototype and annotation process for improvements.
The IQA consisted of validating 12 candidates for every class, covering all classes available.
It was carried out by 11 subjects, who could leave per-class comments through a text box.

\subsubsection{Final Prototype of the Annotation Tool}
The main feedback from the IQA relates to the considerable complexity of the task due to factors such as ambiguity in some class descriptions or the difficulty of annotating sound events with very high inter- and intra-class variation.
The fact that this is found difficult by humans reinforces the idea of manually labelling the dataset instead of using semi-automatic methods.
Based on the insight from the IQA we adopted the following measures to improve the annotation tool and process.
Screenshots of the final prototype can be seen in Figs. \ref{fig:val_task1} and \ref{fig:val_task2}.
\begin{figure}[ht]
%\begin{figure}[ht]
    %\vspace{-4mm}
    \centering
  \centerline{\includegraphics[width=0.50\textwidth]{IEEEtran/figs/sliding_door.png}}
    \caption{Training phase in the annotation tool used for the validation task.}
    \label{fig:val_task1}
    %\vspace{-4mm}
\end{figure}
\begin{figure}[ht]
%\begin{figure}[ht]
    %\vspace{-4mm}
    \centering
  \centerline{\includegraphics[width=0.50\textwidth]{IEEEtran/figs/laughter.png}}
    \caption{Validation phase in the annotation tool used for the validation task.}
    \label{fig:val_task2}
    %\vspace{-4mm}
\end{figure}
\begin{itemize}
    \item Some class descriptions were found ambiguous, allowing multiple interpretations and generating doubts as to the class scope.
    After examining these doubts, we decided to create a list of \textbf{per-class Frequently Asked Questions (FAQs}) to homogenize raters’ judgment and thus gather more consistent annotations (see example in Fig. \ref{fig:val_task1}). The full list of FAQs is provided with the dataset release.
    \item We observed that, in some audio clips, several sound events co-existed with different predominance or salience levels, and this made the ``Present" response rather ambiguous for raters. To address this issue, we decided to \textbf{split the ``Present" response} into ``Present and predominant" (PP) and ``Present but not predominant" (PNP), as specified in Table \ref{tab:responsetypes}.\footnote{Hereafter, we shall use ``Present" to refer to the union of PP and PNP.} A similar approach was used in \cite{salamon2014dataset}. The main motivation for this distinction is to ease the annotation task by mitigating a systematic doubt. But also, this distinction allows to roughly separate a subset of clips containing mostly isolated and clean sound events (PP ratings) vs. others featuring events from several classes and/or in more adverse acoustic conditions (PNP ratings). This could allow defining specific robustness tasks such as training or evaluating with a subset of data of more realistic/adverse conditions, similarly as done in \cite{serizel2020sound} for SED or with ImageNet-A for image recognition \cite{hendrycks2019natural}. In addition, the PP/PNP distinction can be useful for source separation studies \cite{Wisdom_InPrep2020}. We note, however, that this distinction is subjective and these ratings should only be used as a rough indication.
    \item To test the reliability of the submitted responses, we added \textbf{quality control mechanisms} such as the periodic inclusion of verification clips. Whenever the response for one of these clips is wrong, the responses submitted in a given time span are discarded---a common practice in crowdsourcing platforms.
    \item To further ensure high quality annotations, we decided to require \textbf{inter-annotator agreement}. More specifically, each candidate label is presented to several raters until agreement by two different raters on a response type. Once an inter-annotator agreement is reached, the label is considered as \textit{ground-truth} and it is no longer presented to other raters. A similar practice is done in \cite{foster2015chime,cartwright2019sonyc}.
    \item To facilitate the localisation and recognition of sound events within the audio clips, we added the possibility to \textbf{visualize the spectrogram} in addition to the audio waveform, thereby easing the annotation task \cite{cartwright2017seeing}.
    \item We noticed that some audio clips can present highly variable loudness, which can be burdensome (and even harmful) for the rater, and may affect the quality of the annotations. To mitigate this problem, we \textbf{normalize the loudness} of the sound files to some extent following recommendation EBU R-128 \cite{ebu2011loudness}.
    \item To efficiently select which audio clips to present to each rater, we adopt a \textbf{prioritization scheme} that ranks clips according to: \textit{i)} previously rated clips that have not yet reached inter-annotator agreement are prioritized in order to obtain ground truth labels; \textit{ii)} shorter clips are promoted over longer ones as clips with higher label density are considered more useful for learning.
\end{itemize}
Finally, we took two additional measures for the sake of efficiency of the annotation process.
First, the candidates selection in a number of classes had a very bad precision (measured as the percentage of ``Present" responses) due to sub-optimality of the nomination system.
Thus, we decided to discard classes with a rate of ``Not present" responses above 75\%, as well as classes with very few candidates and others deemed highly ambiguous for annotation. 
This left a total of 395 sound classes.
Second, the initial duration limit of 90s was proven burdensome for human validation, and of questionable utility due to the vague supervision given by weak labels applied to such large lengths. Therefore, we decided to discard clips longer than 30s.
These measures meant a significant reduction of the least useful audio data. 
\begin{table*}[]
\centering
\caption{Response types for the validation task.}
%\vspace{0.2cm}
\begin{tabular}{ll}

\textbf{Response type}	    &  \textbf{Meaning}   \\ \hline 
Present and 			&The type of sound described is \textbf{clearly present} and \textbf{predominant}.\\
predominant	(PP)			&This means there are no other types of sound, with the exception of low/mild background noise.\\	
\hline 
Present but not 		&The type of sound described is \textbf{present}, but the audio clip also\\
predominant (PNP)			& \textbf{contains other salient types of sound and/or strong background noise}.\\
\hline 
Not Present	(NP)			&The type of sound described is \textbf{not present} in the audio clip. \\
\hline 
Unsure (U)					&\textbf{I am not sure} whether the type of sound described is present or not.\\
\end{tabular}
\label{tab:responsetypes}
\end{table*}

\subsubsection{Annotation Campaign}
%what
With the final prototype we launched an annotation campaign to validate the candidate labels at scale.
Given that some classes were found much more difficult to annotate than others, we decided to gather annotations using both crowdsourcing and hired raters.
In addition, we divided the classes according to an estimated level of difficulty, based on feedback from the IQA.
%(e.g., ambiguity, familiarity to the non-experienced annotator, etc.).
Table \ref{tab:crowd} lists the annotation strategies adopted for each subset of classes.
\begin{table}[t]
%\vspace{-1mm}
\caption{Annotation strategies adopted for the validation task.}
%\vspace{+3mm}
\centering
\begin{tabular}{ccc}
\toprule
\textbf{class difficulty} & \textbf{classes} & \textbf{annotation strategy} \\
\midrule
easy                    & 77            & crowdsourcing  \& hired annotators          \\
medium                  & 100           & crowdsourcing   \& hired annotators            \\
difficult               & 218           & hired annotators            \\
%\midrule
\bottomrule
\end{tabular}
\label{tab:crowd}
%\vspace{-2mm}
\end{table}
Crowdsourcing consists on gathering validations contributed by any voluntary participant. 
Hence, we made the classes of easy and medium difficulty publicly accessible from FSA.\footnote{\url{https://annotator.freesound.org/fsd/annotate/}}
The most difficult classes, where certain annotation experience was deemed important to provide reliable responses, were kept private.
They were validated by a pool of hired raters who also complemented the crowdsourcing validations in the rest of the classes.

%whooooo, process
In total, over 350 raters contributed, of which six are hired raters and three are the first three authors.
The hired raters consisted of subjects with background in audiovisual engineering, including mostly MSc and PhD students from our research group, with self-reported healthy hearing.
We opted for a small pool of raters in order to have more control on the annotation process and to obtain annotations as consistent as possible.
We recognize this may induce a certain bias in the annotations, but we rather have consistent annotations with agreed bias than a certain lack of consistency likely resulting from crowdsourcing annotations for the difficult classes.
To this end, the hired raters were trained and closely monitored by the first three authors, discussing doubts and agreeing on the best course of action. 
FAQs were gradually extended as more insight was obtained.
Raters were asked to validate groups of related classes (e.g., sibling categories), so they could get familiar with specific sections of the ontology and provide more consistent validations \cite{sabou2014corpus}.
They were instructed to perform the task using high-quality headphones in a quiet environment, and taking periodic breaks to mitigate fatigue.
During the campaign, the hired raters acquired solid expertise on the annotation task and a deep knowledge of the ontology.
Therefore, we consider them experts for this particular task.

%outcome
The outcome of this stage is 51,684 clips considered valid for the dataset, that is, with at least one ``Present" label.
All the ``Present” labels amount to 59,981, all of them being the result of inter-annotator agreement except 3390 which include labels with: \textit{i)} only one PP rating and one PNP rating (and nothing else). This can be considered an inter-annotator agreement at the ``Present” level, attributing the different PP/PNP choice to subjective interpretation; \textit{ii)} only one PP rating (and nothing else); \textit{iii)} only one PNP rating (and nothing else).
The two latter do not meet our definition of ground truth and could be more prone to errors, but were still considered to slightly increase the data.
It must be noted that the set of labels at this point comes from the validation of candidate labels proposed by a simple nomination system, which ultimately relies on the user-provided Freesound tags.
Hence, it is to be expected that some sound events are not covered by the user-generated metadata, or they are not proposed by the nomination system, leading to missing ``Present" labels, a common phenomenon in large sound event datasets \cite{fonseca2020addressing,meire2019impact}.
Therefore, the resulting pool of audio clips have human-validated labels albeit potentially incomplete, which is especially harmful in evaluation.
To address this issue, after splitting the data into development and evaluation sets (Sec. \ref{ssec:split}), the evaluation set is refined using another annotation tool, described in Sec. \ref{ssec:task_gen}.


%============================================================================================
\subsection{Data Split}
\label{ssec:split}
%(0.5)
The input to this stage is a pool of 51,684 audio clips with correct labels in most cases (albeit potentially incomplete).
The goal is to split the data into two subsets: \textit{development} and \textit{evaluation}.
The development set will be used for training and validation.
The evaluation set will be used for system benchmarking after exhaustive annotation.
As stated in Sec. \ref{ssec:design}, the evaluation set is our priority.
A quality evaluation set must be comprehensive, varied, and representative \cite{virtanen2018computational}, while being free from contamination from the development set in order to allow testing models’ generalization capabilities.

\subsubsection{Split Criteria}
We set four criteria for the split.

\textbf{Non-divisibility of uploaders.} The issue of \textit{contamination} must be carefully considered when splitting audio data.
%contamination
It can happen that portions of the data share a common pattern that brings certain acoustic similarity among its constituents.
One typical example is that of ASC, where several recordings are captured in the same physical location for one acoustic scene---therefore, these recordings likely share overall spectral characteristics.
If some of these related recordings are used for training and also for evaluation, their similarity may lead to overly optimistic performance, partly reflecting the ability of the classifier to overfit development examples. As a result, this classifier may suffer from substantial performance drop when tested on new unseen data.
This issue could be called \textit{weak contamination} between development and evaluation.
Note that \textit{weak contamination} should not be confused with \textit{contamination}, which happens when the same (not similar) examples are used for both training and and evaluation (i.e., data leakage).
For simplicity, we will refer to the former simply as \textit{contamination} hereafter.
%We refer to this issue as \textit{contamination} between development and evaluation.
%\footnote{Sometimes it is common to use the term contamination to refer to data leakage---the \textit{same} examples used  for both training and evaluation. Here we relax this statement to merely \textit{similar} examples.}
Recently, this phenomenon was detected in computer vision benchmarks like CIFAR-10 and CIFAR-100 \cite{barz2020we}.
An example of this is regarded as the ``album effect” \cite{whitman2001artist,mandel2005song} or the ``artist effect” \cite{flexer2009album} in music recognition.
Another typical case of contamination happens when a group of clips captured with the same sensor is split in training and evaluation \cite{cartwright2019sonyc}.
To overcome this problem, following the ASC example, a solution is to make sure that all the examples recorded in the same location are placed on the same side of the evaluation (either in development \textit{or} evaluation).
By doing this we promote that the evaluation performance reflects model’s ability to generalize to new audio material and recording conditions.

The case of Freesound audio has some similarities with the above example. 
Audio content in Freesound is uploaded by users, in the following, \textit{uploaders}.
Some uploaders are \textit{small}---they upload a small amount of audio clips---while other uploaders contribute with hundreds of clips.
In the latter case, it can happen that some of the uploaded clips are similar to one another, e.g., several notes of the same music instrument or vocalizations of the same pet. 
When this occurs, we have audio recordings that could share the same sound source and/or physical location and/or recording gear. This could be a source of contamination.
To avoid this issue, we make sure that \textit{all} the content of each uploader is allocated either in the development or evaluation set.
Additional sources of contamination include \textit{i)} audio clip re-purposing (when user $u_a$ downloads a clip by user $u_b$, modifies it, and uploads it as a new clip), and \textit{ii)} the possibility of the same individual creating two user accounts to upload clips.
While these issues were not considered, based on prior experience, they happen rarely and their effect is considered negligible.

\textbf{Small uploaders for evaluation.} 
%Having defined the uploader non-divisibility constraint, selecting a set that is most suited for evaluation implies several axes.
To obtain a varied evaluation set, it seems reasonable to allocate the content from small uploaders as it guarantees a higher diversification of sound sources, acoustic environments and recording gears.
In addition, a closer look at the Freesound data distribution revealed that recordings uploaded by small uploaders tend to be slightly longer.
It can therefore be expected that, in general, these longer recordings tend to contain more sound events when compared to shorter clips---a considerable portion of Freesound consists of relatively short clips often featuring a single event. 
Under this assumption, these longer recordings would be more real-world representative.
Furthermore, this is a more interesting content to annotate exhaustively, and also strongly (i.e., with timestamps) to allow SED evaluation in the future.
Another benefit of using small users for evaluation occurs in the hypothetical worst case scenario of one user uploading very similar clips. In this case, it is likely that a competitive model predicting one of them correctly would also predict correctly all of them, thus generating a fake performance resolution. By selecting small users we mitigate this problem.

\textbf{A coarse class distribution is enough.} A fine-level split carefully matching a given class distribution is not needed at this point, as during the exhaustive annotation of the evaluation set we expect some classes to grow. This will create an imbalance that will need to be compensated.
% Beyond promoting the allocation of non-divisible small uploaders,

\textbf{Focus on leave nodes.} Among the classes available at this point, we focus on the subset of 113 leaf nodes with more than 100 clips as they are considered the most important classes.




%-----------
\subsubsection{Split Method}
Given the many constraints, off-the-shelf methods such as random sampling, iterative stratification \cite{sechidis2011stratification} or combinatorial optimization algorithms like knapsack problems \cite{toth1990knapsack} are not well suited.
Therefore, we implement an \textit{ad hoc} approach consisting of iteratively allocating uploaders' content to the evaluation set after sorting them appropriately.
%algo
First, we compute a score per uploader $u$ as:
%\ref{eqn:score_eval}
\begin{equation}
score^u = n\_labels_{max}^u + \frac{1}{K_u} \sum_{k=1}^{K_u} n\_labels_{c_{k}}^u,
\label{eqn:score_eval}
%\vspace{-1mm}
\end{equation}
where the first term $n\_labels_{max}^u$ represents the maximum number of labels provided by the uploader $u$ in any class, $n\_labels_{c_{k}}^u$ represents the number of labels provided by $u$ in the class $c_{k}$, and $K_u$ is the number of classes \textit{touched} by $u$.
Uploaders are sorted in ascending score order and the content of low-score uploaders are transferred first.
In this way, with the first term we prevent uploaders with abundant content concentrated in one specific class and with the second term preference is given to users with low average number of labels per class for higher diversity.
% accounting for the scattering of $u$ across classes.
Upon inspection of the top-ranked uploaders, we found out that by splitting the target 113 leaf nodes, some content associated with the remaining classes is also automatically allocated due to the scattering of uploaders across various classes.
The amount of this additional content is deemed sufficient, given that a fine-level class distribution is not the goal at this point.
We then proceed to allocate data to the evaluation set. 
A pseudocode version of the process is shown in Algorithm \ref{alg:eval_split}.
\begin{algorithm}[h]
\DontPrintSemicolon
\SetAlgoLined
\KwData{Empty evaluation set per-class $E=\left\lbrace e_{c_{i}}=0 \right\rbrace_{i=1}^C$, uploaders ranking $\boldsymbol{u}$}
 %initialization\;
 %\For{pass $n = 1,2, \dotsc  N $}{
    \For{class $c_i \in C$}{
      get current evaluation target $t_{c_{i}}$ \;
      \While{$e_{c_{i}} < t_{c_{i}}$}{
        get next uploader $u$ in ranking $\boldsymbol{u}$ with data  in $c_{i}$\;
        $e_{c_{i}} \leftarrow e_{c_{i}}$ + data from $u$ in $c_{i}$ \;
         \For{class $c_k \in K_u$}{
            $e_{c_{k}} \leftarrow e_{c_{k}}$ + data from $u$ in $c_{k}$ \;
        }
      }
    }
 %}
 \KwResult{A candidate evaluation set}
 \caption{Data allocation to evaluation set}
 \label{alg:eval_split}
\end{algorithm}

We traverse the $C=113$ classes starting from the least-represented ones since they have less flexibility for data allocation.
For each class, we progressively allocate content from the ranked uploaders until a target amount of data is reached.
This target ranges from 50 to 100 labels per class, depending on total class label count.
By default, the maximum uploader size per class is set to 10\% of the evaluation set.
Thanks to the proposed sorting, uploaders in the evaluation set do not reach such a maximum in the majority of classes (in many occasions they provide one single clip)---if they do, excess clips are discarded in most cases.
However, due to the very high uploader diversity, the maximum uploader size had to be increased in a few exceptions.
Likewise, some uploaders were considered inadequate for evaluation and were manually assigned to development.
Using the proposed scheme, we process all the 7229 uploaders and we allocate 2794 of them to the evaluation set, totalling 11,466 clips.

The outcome is two pools of audio clips disjoint in terms of uploaders: a candidate development set and a candidate evaluation set. The latter is exhaustively labeled in the refinement task.


%============================================================================================
\subsection{Refinement Task}
\label{ssec:task_gen}
%(0.5)
%motivation - goal
As mentioned in Sec. \ref{ssec:task_val}, in some clips, the current label sets could be an underrepresentation of the audio content, biased by the idiosyncrasies of the labeling pipeline.
%Why missing labels are dangerous in eval? Had the current label sets were used for evaluation, in some cases, 
This is especially harmful in evaluation, as classifiers would be penalized when predicting a correct label that happens to be missing from the ground truth.
This critical issue would limit the utility of the dataset for system's benchmarking.
To address this issue, we refine the labels in the evaluation set.
The goal is to obtain an \textit{exhaustive} labelling, that is, a labelling as close as possible to the correct and complete transcription of the audio content (for the considered vocabulary of 395 classes).

\subsubsection{Annotation Tool}
To achieve this goal, we designed and implemented an annotation tool that allows two subtasks:
\textit{i)} to review the existing labels, and \textit{ii)} to add missing ``Present" labels.
%this poses a problem
The second subtask, in particular, has a considerable complexity since audio clips can sometimes contain totally unrelated sound events.
Therefore, the success of this task relies on two key factors: \textit{i)} raters with a deep understanding of the ontology, the agreed FAQs, and the particularities of the audio material; \textit{ii)} an interface that facilitates exploration of the large vocabulary of the ontology.
%who
In regard to the first factor we turn to the pool of hired raters (4 of the initial 6), who acquired a solid expertise by extensive participation in the validation task (\ref{ssec:task_val}), hence they are considered experts for this purpose.
% task/process
As for the second factor, the refinement task (also deployed in FSA) features an interactive table where raters can easily explore different depth levels of the ontology (see Fig. \ref{fig:ref_task2}). 
\begin{figure}[ht]
%\begin{figure}[ht]
    %\vspace{-4mm}
    \centering
  \centerline{\includegraphics[width=0.50\textwidth]{IEEEtran/figs/f3.png}}
    \caption{Table for exploring the ontology in the annotation tool for the refinement task.}
    \label{fig:ref_task2}
    %\vspace{-4mm}
\end{figure}
This tool is based on a previous version described in \cite{favory2018facilitating}.
A text-based search allows to quickly navigate to classes in the table, where their hierarchical context is shown.
For each class, textual descriptions and representative sound examples are displayed.
The interface facilitates the comparison of different classes by simultaneously displaying their information.
%, which was found very useful.

\subsubsection{Annotation Process}
Clips were presented grouped by sound class to facilitate the task. For every class:
\begin{enumerate}
    \item raters were instructed to go through a \textbf{training phase} (same as in the validation task---see Fig. \ref{fig:val_task1}). 
    \item For every clip, they would first \textbf{review the existing labels} displayed and modify them if needed. Then, they were instructed to \textbf{add any missing labels} by exploring the ontology (Fig. \ref{fig:ref_task2}).
\end{enumerate}
While reviewing/adding labels, they were instructed to provide the most specific labels possible (typically leaf labels) as this is the richest supervision.
The quality practices described in Sec. \ref{ssec:task_val} for the validation task also apply here.
%Like in the validation task, the raters were closely monitored by the first three authors.
Following this procedure, each evaluation label was verified or reviewed by between two and five independent annotators (considering both validation and refinement tasks), including at least one expert.
As a result, annotations are expected to be correct and complete in the vast majority of cases.
The exhaustive labelling carried out has two implications.
First, absence of labels means absence of sound events (except human error)---a desired feature.
Second, some classes are now much more represented than before as they are prevalent but were underrepresented, thereby creating a class imbalance.

The outcome of this stage is a pool of exhaustively labeled clips (for the considered vocabulary), the majority of which will form the evaluation set.

%============================================================================================
\subsection{Post-processing}
\label{ssec:postpro}
%(1)
%The goal of this stage is to post-process the incoming pools of data in order to finalize the proposed dataset FSD50K.
This stage starts from two sets of data: a candidate development set with correct but potentially incomplete labels, and an exhaustively-labeled candidate evaluation set.
The vocabulary used so far comprises 395 classes, yet many of them have few data (in the range of few tens of clips).
While they are not adequate for common machine learning standards (e.g., deep learning), they can be useful for other practices requiring less data (e.g., few shot learning \cite{cheng2019multi}) or for creative purposes beyond machine learning.
Likewise, this information can provide insight as to the specific content of the dataset.
Therefore, we provide two different formats for the annotations in FSD50K: 
\begin{enumerate}
    \item The raw outcome of the annotation process, featuring all generated class labels without any restriction. These include classes with few data. We call this the sound \textit{collection} format and encompasses a vocabulary of 395 classes.
    \item The outcome of curating the raw annotations into a machine learning dataset with emphasis in sound event recognition tasks. This process involves, mainly, merging low prior classes into their parents thus ensuring a minimum amount of per-class data. This is the \textit{ground truth} for FSD50K, with a vocabulary of 200 classes.
\end{enumerate}
Next, we explain the post-processing carried out to obtain FSD50K (consisting of a set of audio clips and the corresponding ground truth).
Further details about both aforementioned formats can be found in FSD50K's Zenodo page.\textsuperscript{\ref{foot_zenodo}}


\subsubsection{Determine FSD50K vocabulary}
%We define valid leaf nodes as those with at least 100 clips, and without an extreme development/evaluation imbalance. 
We define valid leaf nodes as those meeting two requirements: a minimum of 100 clips, and without extreme development/evaluation imbalance. 
This is a trade-off between abundant per-class data and preserving a lot of leaf nodes.\footnote{Given the particularities of some classes, the requirements to consider a leaf node valid are relaxed in a few exceptions.} We take the following measures.

\textbf{Merge non-valid leaf nodes with their parents.}
%First, non-valid leaf nodes are merged with their parents. 
There are two variants of this process, depending on the type of branch in the hierarchy.
First, non-valid siblings of valid leaf nodes are merged with their parents.
In these branches, the level of specificity is fixed by the valid sibling.
For instance, \textit{Yip}, a class with few data which is sibling of \textit{Bark} and child of \textit{Dog}, is merged with \textit{Dog} and the most specific label in this branch is the valid leaf \textit{Bark}.
Then, in branches without any valid leaf nodes, all leaf nodes are merged with their parents, which in turn become new leaf nodes (since they no longer have children).
This process is repeated recursively, pruning the branch by moving upwards in the hierarchy, until a new leaf node becomes valid.
Ideally, we want to prune the branches as little as possible to preserve the most specific (and informative) nodes.
However, due to data scarcity, sometimes low-level nodes are inevitably merged with non-specific parents, e.g., \textit{Domestic sounds, home sounds}.

The minimum data requirement is enforced at the leaf node of every branch.
However, the requirement is not enforced in its ancestors, which are intrinsically valid because the leaf node provides enough data. This means that, occasionally, the data explicitly associated with one ancestor may be scarce. For example, \textit{Rail transport} is a valid intermediate node despite it holding very few data, because their children (\textit{Train} and \textit{Subway, metro, underground}) are valid, holding most of the data in this branch. This is a result of the nomination system and annotation processes, that favour more specific labels.

\textbf{Remove some valid leaf nodes to obtain a more semantically consistent vocabulary.}
%Second, we remove some valid leaf nodes to obtain a more semantically consistent vocabulary.
As a result of the pruning, some parents with various children in the ontology end up having very few in the candidate dataset, either due to data scarcity or to extreme imbalance.
In most cases, this is not a problem as children are rather independent semantically---e.g., \textit{Domestic sounds, home sounds} encompasses 27 children that occur usually in domestic environments but with weak semantic links otherwise.
However, in other cases, children constitute a pre-established subset of closely related classes that makes more sense when all of them co-exist. 
This is the case, for instance, of the classes \textit{Light engine (high frequency)}, \textit{Medium engine (mid frequency)}, and \textit{Heavy engine (low frequency)}, where only the former is valid.
Thinking on the real operation of models trained on FSD50K, the fact that only one of these children is valid could potentially lead to unnatural predictions biased by the choice of the vocabulary, i.e., recurrently spiking \textit{Light engine (high frequency)}, absent their complementary siblings.
To prevent this issue, we merge some ``isolated" valid leaf nodes with their parents, thus obtaining a more semantically consistent vocabulary. 
%Apart from the mentioned engine types, this also occurs with wind and bowed string instruments.
Hence, despite having a substantial number of, e.g., light engine and saxophone sounds, they are not part of the vocabulary---only \textit{Engine} and \textit{Wind instrument, woodwind instrument} are. Note however that these more specific annotations are indeed available in the sound collection format.

\textbf{Discard some non-essential intermediate nodes.}
%Lastly, we discard some non-essential intermediate nodes:
This includes classes of abstract nature or nodes with ambiguous children providing few data, e.g., \textit{Digestive} or \textit{Arrow}, respectively. The outcome is a vocabulary of 200 classes (144 leaf nodes and 56 intermediate nodes).

\subsubsection{Balancing development/evaluation sets}
%=========================================================================
As a result of exhaustive labelling the evaluation set, the proportion of some frequently occurring sound events arose substantially, sometimes even surpassing the amount of labels in the development set.
To address this issue, we first identified a set of 40 leaf nodes which benefit from transferring data from evaluation to development.
Then, we selected a portion of 1182 evaluation clips such that: \textit{i)} their evaluation content encompasses the 40 target classes while the impact on the remaining ones is minimal (note the multilabel nature of the clips); \textit{ii)} they are disjoint from the remaining set of clips in terms of uploaders, as explained in Sec. \ref{ssec:split}.
%Experiments were carried out to confirm that this data removal did not cause any pathological issue on the sound classes.
The outcome of this data transfer is an evaluation set of 10,231 clips, and a per-class development/evaluation proportion ranging from 50/50\% to 75/25\% in the vast majority of leaf nodes.
The per-class split proportion depends on factors like data availability, ubiquity of the sound events, degree of multilabelness of the audio clips, and non-divisibility of content from the same uploader.
Exceptions include \textit{Chatter}, \textit{Chirp, tweet} and \textit{Male speech, man speaking}, for which there are more evaluation labels than development labels due to the exhaustive annotation of these ubiquitous sound events.
In addition to shaping the evaluation set, with this data transfer we make available some exhaustively labeled content for validation.


%=========================================================================
\subsubsection{Validation Set}
Some recent large audio datasets do not provide predefined validation sets \cite{gemmeke2017audio,Mesaros2018_DCASE} allowing dataset users to create their own according to their preferences.
Nonetheless, for easier dataset consumption and to facilitate reproducibility we propose a candidate split of the development set into train and validation sets.
We consider that a validation set should ideally meet the following requirements:
\begin{itemize}
    \item \textbf{Proportion}. The validation set should amount to a specified proportion of the development set, typically between 10 and 20\%. Note that due to the multilabel and variable-length nature of Freesound audio, the proportion can be different in terms of audio clips, labels, and duration.
    \item \textbf{Stratification}. The class label distribution should be similar in both train and validation sets.
    %, that is, the frequency of occurrence of each label is roughly preserved between both sets.
    \item \textbf{Contamination}. As explained in Sec. \ref{ssec:split}, contamination across splits should be minimized.
\end{itemize}
Unfortunately, due to several practical constraints, these requirements can not always be met, and our case is not an exception.

Typical ways to make train/validation splits of multilabel data include random sampling or iterative stratification \cite{sechidis2011stratification}.
Both methods can produce desired data proportions and class distributions, iterative stratification being a common option for multilabel data.\footnote{Random sampling does not account for stratification per se, but a workaround is to compute many train/validation splits and choose the one that minimizes a distance between the respective class distributions.} 
However, they fail to keep non-divisibility of content from the same uploader, thus generating contamination.
The distribution of number of clips contributed by uploader is very varied in our development set, with some uploaders contributing very few clips in very few classes while others contribute hundreds of clips scattered across many classes. 
In addition, because we already allocated a large amount of small uploaders into the evaluation set (Sec. \ref{ssec:split}), preserving uploader non-divisibility at this point means deviating from the target class distribution.
In other words, it is difficult to strictly meet the three above requirements simultaneously, and therefore we need to relax their application.

We focus on the contamination requirement.
After closely inspecting the data, we distinguish two types of contamination: \textit{i)} \textit{within-class} (WC) contamination, which happens when content from the same uploader \textit{and} belonging to the same class is placed at both train and validation sets;
\textit{ii)} \textit{between-class} (BC) contamination, which occurs when content from the same uploader \textit{but not} from the same class is placed at both train and validation sets.
We hypothesize WC contamination is more harmful as it could imply having the same sound source, physical location and/or recording gear in both sets. 
By contrast, BC would have less impact as, in most cases, the acoustic material would be different, and also possibly the acoustic environment.
Under this hypothesis, we build the validation set focusing on minimizing WC contamination but being flexible with the BC one.
To do this, we employ a method similar to that of Sec. \ref{ssec:split}, but tailored to this specific problem.
We first define the content from one uploader labeled with the same class label as the minimum non-divisible entity whose entirety should be preserved.
Then, we adopt an iterative process in which, after sorting the uploaders per-class according to a given criteria, we progressively allocate their content to the validation set.
We describe the method in detail next.


As preprocessing, we first initialize the validation set with most of the data transferred from evaluation to development in the previous stage---this content is well suited for evaluation purposes as it is  exhaustively labeled. 
We then compute a score per uploader per class. 
The score for a user, $u$, in the class $c_i$ is given by:
%\ref{eqn:score_val}
\begin{equation}
score_{c_{i}}^u = \alpha n\_labels_{c_{i}}^u + \beta \frac{1}{K_u} \sum_{k=1}^{K_u} n\_labels_{c_{k}}^u,
\label{eqn:score_val}
%\vspace{-1mm}
\end{equation}
where $n\_labels_{c_{i}}^u$ represents the number of labels provided by the uploader $u$ in the class $c_{i}$, $K_u$ is the number of classes \textit{touched} by $u$, and $\alpha$ and $\beta$ are tunable weights to set the relevance of each term, both $\in [0,1]$.
The first term represents the amount of data in the class $c_{i}$ by $u$, whereas the second term is the average number of labels per class, accounting for the scattering of $u$ across classes.
The score is inversely proportional to suitability for validation---uploaders are sorted in ascending score order and the content of low-score uploaders are transferred first.
By tuning $\alpha$ and $\beta$ we aim to promote first the uploaders providing a small amount of data in the class under question, $c_{i}$, with minimal or no scattering. 
This facilitates adjustment to a target class distribution while minimizing contamination (both WC and BC).
This first group of uploaders is followed by others with smooth scattering across classes, avoiding uploaders with large contributions concentrated in specific classes.
This again facilitates adjusting to a target distribution while minimizing the need to split content from the same uploader in one class (i.e., WC contamination), but allowing BC contamination.

Once the validation set is initialized and the uploaders are sorted per-class, we proceed to allocate data to the validation set. A pseudocode version of the process is shown in Algorithm \ref{alg:val_split}.
\begin{algorithm}[h]
\DontPrintSemicolon
\SetAlgoLined
\KwData{Initialized validation data per-class $V=\left\lbrace v_{c_{i}} \right\rbrace_{i=1}^C$, uploaders ranking in development set per-class $U=\left\lbrace \boldsymbol{u_{c_{i}}} \right\rbrace_{i=1}^C$}
 %initialization\;
 \For{pass $n = 1,2, \dotsc  N $}{
    \For{class $c_i \in C$}{
      get current validation target $t_{c_{i}}$ \;
      \While{$v_{c_{i}} < t_{c_{i}}$}{
        get next uploader $u$ in ranking $\boldsymbol{u_{c_{i}}}$ \;
        $v_{c_{i}} \leftarrow v_{c_{i}}$ + data from $u$ in $c_{i}$ \;
        \If{data is multilabel to class $c_j$}{
           $v_{c_{j}} \leftarrow v_{c_{j}}$ + data from $u$ in $c_{j}$ \;
        }
      }
    }
 }
 \KwResult{A candidate validation set}
 \caption{Data allocation to validation set}
 \label{alg:val_split}
\end{algorithm}
We traverse the classes in several passes, and, for each class, we progressively allocate content from the ranked uploaders until a target amount of data is reached.
Note that when separating the class $c_i$, the algorithm does not care that a given uploader $u$ contributes to another class $c_j$ (BC contamination), unless there is at least one audio clip that bears class labels for both classes $c_i$ and $c_j$.
WC contamination can be produced in the steps corresponding to lines 6 and 8.
For example, we designed the step of line 6 so that, if adding the content from one uploader implies exceeding the validation target, $t_{c_{i}}$, by more than 15\%, two things can happen.
If the current validation amount is $v_{c_{i}} > 0.75 t_{c_{i}}$, the content is not transferred, $v_{c_{i}}$ is considered sufficient, and the procedure is halted for class $c_i$. 
This flexibility allows to minimize WC contamination at the expense of deteriorating stratification.
Otherwise, if $v_{c_{i}} <= 0.75 t_{c_{i}}$, the content from $u$ in $c_i$ is split and the amount needed to reach $t_{c_{i}}$ is allocated, causing WC contamination. 
Similar heuristics are adopted for the step in line 8.

Using the proposed scheme, we process clips from the 4936 uploaders in the development set.
Due to the high variability of users, the process needs initial babysitting with a subset of classes in order to tune the weights $\alpha$ and $\beta$ to our problem. 
We finally use $\alpha=0.4$ and $\beta=0$ when a user contributes only to one class, and $\alpha=0.3$ and $\beta=0.7$ otherwise.
Using several passes (instead of one) allows us to better adjust the class distribution. 
We use $N=2$ passes starting from classes in need of more validation data, which allows us to reach a reasonable stratification. 
The target validation proportion is 15\% of the development labels per-class, except for the largest 17 classes where we reduced this percentage progressively (as we considered that enough data was allocated).
The first-pass target is to fill 60\% of the final target (i.e., $0.6\cdot15\% = 9\%$).
The second-pass target is the final target ($15\%$).
We only consider the leaf nodes for this process ($C=144$).
This is done for simplicity and because the leaf nodes are the most specific data that will receive labels from the rest of the ontology levels upon label propagation to their ancestors.
In this way, validation data at all levels of the ontology is guaranteed.

The outcome is a validation set which represents a tradeoff between stratification and contamination.
%It is composed of 4170 audio clips (of which 158 do not have leaf labels, and ended up due to the step of line 8 in Algorithm 1 (multilabel nature to non-leaf nodes).
Composed of 4170 audio clips, it amounts to 13.3\% of the content associated with leaf nodes and 10.2\% of the entire development set.
The main stats for this candidate validation set are listed in Table~\ref{tab:val_set}.
\begin{table}[ht]
%\vspace{-1mm}
\caption{Main stats for candidate validation set.}
%\vspace{+3mm}
\centering
\begin{tabular}{cccc}
\toprule
\textbf{clips} & \textbf{duration} & \textbf{uploaders} \\
\midrule
4170             & 9.9h           & 2224           \\
%\midrule
\bottomrule
\end{tabular}
\label{tab:val_set}
%\vspace{-2mm}
\end{table}
Out of the 2224 uploaders with content in the validation set, 641 also have content in the train set. Note, however, that most of these cases correspond to BC contamination.
Sec. \ref{ssec:exp_val} includes a set of experiments to demonstrate the efficacy of the proposed method for train/validation separation, comparing it to other separation methods.
As described, this candidate train/validation split is the result of a number of design choices.
Depending on user preferences and/or end applications, other choices may be desirable in terms of proportion, contamination, usage of leaves vs. intermediate nodes, etc.
For this reason, FSD50K provides uploader information as part of the additional metadata, allowing dataset users to create alternative validation sets.


\subsubsection{Ground Truth Hierarchical Propagation}
%=========================================================================
The human-provided labels at this point are usually from classes corresponding to lower levels of the ontology, especially for the evaluation set (see Sec. \ref{ssec:task_gen}).
This occurs due to two reasons: \textit{i)} the uploader-provided tags used in the nomination system are naturally lower-level concepts (\textit{Meow}, \textit{Cat}) rather than higher-level ones (\textit{Animal}); 
\textit{ii)} in the refinement task, annotators were instructed to generate labels as specific as possible.
In order to obtain an exhaustive labelling hierarchy-wise, we need to propagate the current labels in the upwards direction to the root of the ontology, determining the ancestors in the hierarchical path and automatically assigning them to the corresponding audio clips.
This label propagation process is sometimes referred to as \textit{label smearing} \cite{gao2017knowledge}.

In most cases, label smearing is a straightforward process as there is one single unequivocal path from a given low-level node to the root.
However, in other cases, nodes and root are connected by more than one path.
Among these multiple-path cases, some have all the paths valid by default according to the semantics of the node.
This allows straightforward propagation as in the single-path case, e.g., \textit{Doorbell} can be directly propagated to \textit{Door} and \textit{Alarm}.
However, in the majority of cases, only a subset of the paths is valid (typically one), or even none of the paths is valid by default due to the parents-node relationship. For instance, \textit{Buzz} cannot be directly propagated to its parents \textit{Fly, housefly} or \textit{Bee, wasp, etc.} unless we have explicit information about the source of the buzz sound. 
In these cases, we need knowledge of the correct immediate parent(s) to unambiguously infer ancestors for a complete hierarchical labelling.
Parents disambiguation can be carried out in different ways depending on the annotation task.
In the clips annotated only with the validation task, the disambiguating parents will exist iff the nomination system proposed them.
For the clips annotated also with the refinement task, raters were instructed to specify the disambiguating parents when needed; however, 
%this additional annotation subtask is an added complexity that rarely happens, which makes it prone to errors. Upon inspection of the gathered annotations, 
we detected that they were not always specified.

As a result, in these cases, ancestors cannot be inferred from the leaf node, leading to hierarchical paths featuring missing parts.
For example, \textit{Growling} is connected directly to \textit{Animal} in several cases where information of the source animal is not available.
The policy followed in case of ambiguous ancestors was to not include these labels (hence potentially creating missing “Present” labels in the mid- or high-levels of the ontology) instead of possibly generating incorrect labels.
In the development set, these cases are provided as is since it is less critical. 
By contrast, because the cases in the evaluation set are more critical, they were partially reviewed and corrected. 
The potential impact of missing intermediate nodes is restricted to some instances of class labels with multiple-paths where the disambiguating parents could not be determined, and thus we expect this to have a minimal impact.

To finalize the label smearing process we filter out the out-of-vocabulary labels (labels beyond the 200 selected). In the majority of cases, these correspond to abstract or blacklisted classes. This is another reason why some clips have labels up to the ontology root while others only have a portion of it or even one single label. For example, \textit{Whoosh, swoosh, swish} has no hierarchy as all class labels in its path were either removed previously due to specified constraints (\textit{Arrow}) or removed in this last step (as classes above \textit{Arrow} are abstract). This can be easily spotted in the provided ground truth CSV files.
The number of labels before/after the propagation process can be seen in Table~\ref{tab:main_stats} (\textit{unpropagated} and \textit{smeared}, respectively).
The outcome is a set of \textit{smeared} labels consistently encompassing all relevant levels of the ontology.
%, through upwards propagation of the initially human-provided lower-level class labels. 
Note the considerable increase of labels, despite we are ignoring parts of the ontology. This is the ground truth provided for FSD50K.


==> S4_Description.tex <==
FSD50K is an open dataset of human-labeled sound events containing 51,197 audio clips unequally distributed in 200 classes drawn from the AudioSet Ontology. 
This Section discusses its main characteristics, limitations and applications.
The dataset is freely available with both clips and metadata released under CC licenses, and can be downloaded from Zenodo.\textsuperscript{\ref{foot_zenodo}}
In the following, we refer to development, training, validation and evaluation sets described in the previous Sections as \textit{dev}, \textit{train}, \textit{val}, and \textit{eval}.

%============================================================================================
\subsection{Characteristics}
\label{ssec:characteristics}

%content, classes, leaves nodes
FSD50K is composed mainly of sound events produced by physical sound sources and production mechanisms.
Hence, the main focus is on the \textit{casual listening} perspective of sound, as defined by Schaeffer \cite{schaeffer2016traite}).
It also includes some classes that can inherently encompass several more specific sources (\textit{Train}), some classes that do not relate to a specific source but to the perception of sound (\textit{Clatter}), and few abstract classes (\textit{Human group actions}).
The dataset has 200 sound classes (144 leaf nodes and 56 intermediate nodes) hierarchically organized with a subset of the AudioSet Ontology \cite{gemmeke2017audio}.
Note, however, that in some cases one leaf node in FSD50K (\textit{Camera}) may be an intermediate node in AudioSet due to the merge of low prior classes (\textit{Single-lens reflex camera}) with their parents (Sec. \ref{ssec:postpro}).
Following the main families in the AudioSet Ontology, the FSD50K vocabulary encompasses mainly \textit{Human sounds}, \textit{Sounds of things}, \textit{Animal}, \textit{Natural sounds} and \textit{Music}.
%, as well as a few classes belonging to \textit{Onomatopoeia} and \textit{Deformable shell}.
The vast majority of the content corresponds to recorded sounds, while a small portion corresponds to sounds generated with devices, typically in the context of musical instruments, e.g., some bass drums are generated with drum machines.

%clips, labels, duration
The main characteristics of FSD50K in terms of number of clips, labels, duration and uploaders are listed in Table~\ref{tab:main_stats}.
\begin{table}[ht]
%\vspace{-1mm}
\caption{Main stats for FSD50K}
%\vspace{+3mm}
\centering
\begin{tabular}{lccc}
\toprule
             & \textbf{total} & \textbf{dev} & \textbf{eval} \\
\midrule
clips            & 51,197         & 40,966 (80\%)          & 10,231 (20\%)        \\
labels (unpropagated)  & 62,657         & 45,607 (72.8\%)        & 17,050 (27.2\%)      \\
avg labels/clip      & 1.22           & 1.11             & 1.67 \\
labels (smeared) & 152,867        & 114,271              & 38,596       \\
clips w/ leaf label(s)          & 40,461           & 31,310               & 9151      \\
duration         & 108.3h         & 80.4h (74.2\%)          & 27.9h (25.8\%)  \\
avg duration/clip    & 7.6s           & 7.1s             & 9.8s  \\
uploaders          & 7225           & 4936               & 2289      \\
%\midrule
\bottomrule
\end{tabular}
\label{tab:main_stats}
%\vspace{-2mm}
\end{table}
\begin{figure*}[h]
        \centering
        \begin{subfigure}[b]{0.475\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{IEEEtran/figs/barh_labels_dev.pdf}
            \caption{Label distribution in dev}
            \label{fig:label_dev}
        \end{subfigure}
        %\quad
        \begin{subfigure}[b]{0.475\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{IEEEtran/figs/barh_labels_eval.pdf}
            \caption{Label distribution in eval}
            \label{fig:label_eval}
        \end{subfigure}
        %\vskip\baselineskip
        \begin{subfigure}[b]{0.475\textwidth}
            \centering
            \includegraphics[width=\textwidth]{IEEEtran/figs/histo_length_dev.pdf}
            \caption{Clip length distribution in dev}
            \label{fig:clip_len_dev}
        \end{subfigure}
        %\hfill
        \begin{subfigure}[b]{0.475\textwidth}  
            \centering 
            \includegraphics[width=\textwidth]{IEEEtran/figs/histo_length_eval.pdf}
            \caption{Clip length distribution in eval}
            \label{fig:clip_len_eval}
        \end{subfigure}
        \caption[]
        {\small Distributions of audio clip lengths and labels for dev and eval. Clips in eval tend to last slightly longer (by dataset design) and have more labels (by dataset curation). Bins in (a,b) correspond to 1/3 second. Xaxis scale in (c,d) is logarithmic. Number of labels is reported in the \textit{unpropagated} form. Note visualization span differ among plots.} 
        \label{fig:dataset_plots2x2}
\end{figure*}
The audio clips are grouped into a dev split and an eval split such that they do not have clips from the same uploader.
%The dataset is constructed emphasizing the diversity of eval, via inclusion of a higher variety of small uploaders.
Eval is exhaustively labeled, that is, annotations are correct and complete for the considered vocabulary.
In dev, a small amount of content is exhaustively labeled, but the vast majority is composed of labels that are correct but could be occasionally incomplete due to the validation task processing (Sec. \ref{ssec:task_val}).
The number of labels is expressed in \textit{unpropagated} and \textit{smeared} forms.
The number of unpropagated labels includes only the most specific labels per clip.
It must be noted that this way of counting labels ignores a few labels in cases where a sound event co-occurs with: \textit{i)} events from low prior siblings that were merged with their parent; \textit{ii)} events that do not fit semantically in any other sibling provided by the ontology, hence they are annotated with their parent.
While these cases are not frequent, the true number of human-provided labels describing sound events would be slightly larger than the one reported here.
Smeared labels refer to the labels after hierarchical propagation (Sec. \ref{ssec:postpro}).
We use the unpropagated version to compute the average number of labels per clip.
Note the increased amount of labels per clip in eval due to the exhaustive labelling process, as can also be seen by comparing the label distributions in Figs. \ref{fig:label_dev} and \ref{fig:label_eval}.
A total of 31,310 clips are labeled with, at least, one leaf label in dev---the remaining 9656 clips are labeled only with intermediate node labels.
This proportion changes significantly in eval, where the majority of clips have leaf labels (9151 out of 10,231)---this is due to the label specificity policy used in the refinement task (Sec. \ref{ssec:task_gen}).
All labels in the provided ground truth are smeared, i.e., consistently propagated to their ancestors in the hierarchy.
PP/PNP annotations are provided for the labels validated in the validation task.
Out of the 108.3 hours of human-labeled audio, 31.5 are exhaustively labelled, most of them used for evaluation purposes (eval and val).
The audio clips are of variable length ranging from 0.3 to 30s.
Note the increased average duration of eval clips, due to the allocation process (Sec. \ref{ssec:split}), which can also be noticed by comparing the audio clip length distributions in Figs. \ref{fig:clip_len_dev} and \ref{fig:clip_len_eval}.
The ground truth labels are provided at the clip-level (i.e., weak labels).
The dataset is nourished from 7225 Freesound users and the content was uploaded from the launch of Freesound in 2005 until the beginning of 2019.
%-------end of table

% classes and data
The number of clips per leaf class varies, roughly, from 40 to 200 in eval, and from 50 to 500 in dev, with a few exceptions.
The number of clips in the intermediate nodes grows much more depending on the hierarchy.
Therefore, class imbalance comes from two sources: non-uniform class distribution and variable-length of clips.
%format
The dataset is licensed under CC-BY license---nonetheless, each clip has its own specific license (all of them CC). 
All clips are provided as uncompressed PCM 16 bit 44.1 kHz mono audio files.
Further details about data licenses, ground truth format, and additional provided metadata can be found in the FSD50K Zenodo page.\textsuperscript{\ref{foot_zenodo}}

 

%-duration per class. cuales son las clases con clips mas largos. por que? son outdoor? box plot
%-per-class results to show classes


    

%============================================================================================
\subsection{Discussion}
\label{ssec:discussion}

\subsubsection{Variable Clip Length and Label Weakness}
Labels in FSD50K are provided at the clip-level (i.e., weak labels).
However, unlike other sound event datasets featuring audio clips of (quasi-) constant length (e.g., \cite{gemmeke2017audio,salamon2014dataset,salamon2017scaper}), FSD50K is composed of variable-length clips in the range [0.3, 30] seconds (see Figs. \ref{fig:clip_len_dev} and \ref{fig:clip_len_eval}).
This provides FSD50K with a particular feature.
On the one hand, it is not uncommon that clips contain sound events where the acoustic signal fills almost the entirety of the file, which can be understood as strong labels.
To give a sense of how frequent this is, 12,357 clips in the dev set are shorter than 4s and bear one single label validated only with PP ratings.
Thus, we estimate that the dev set is composed mainly of weakly labeled data and a portion of strongly labeled data, in a rough proportion of 70\%/30\%.
On the other hand, another small portion of the data presents a much weaker supervision---e.g., 9494 dev clips are longer than 10s (see Fig. \ref{fig:clip_len_dev}).
In these longer clips, lower label densities lead to higher label noise since there is less  certainty of where the event is actually happening, sometimes referred to as \textit{label density noise} \cite{shah2018closer}.
The impact and limitations of weak labels in SER are discussed in \cite{turpault2020limitations,Fonseca2019learning}.
In the context of deep networks, clips' variable length implies that audio processing must be done either using fixed-length patches or utilizing variable-length inputs.
The former approach implies two issues: \textit{i)} in training, the weak labels must be inherited by every patch (a practice called \textit{false strong labeling} in \cite{morfi2018data}), which can generate false positives if the label is not active in a given patch---which is more likely to happen as the clip gets longer;
\textit{ii)} in evaluation, patch-level scores must be aggregated into clip-level scores to evaluate clip-level predictions against the weak labels.
The latter approach is free from the mentioned nuisances, but entails certain architectural constraints, such as using fully convolutional networks or appropriate pooling strategies.

\subsubsection{Audio Quality}
Given the high diversity of Freesound audio (Sec. \ref{ssec:acqui}), it is difficult to make strong claims about audio quality in FSD50K.
Nonetheless, upon inspection of the clips' metadata (e.g., inspecting the tag cloud in Freesound), it can be seen that many Freesound users utilize (semi-) professional recording equipment (e.g., microphones, A/D converters or preamplifiers of brands such as \textit{Neumann}, \textit{Rode} or \textit{Tascam}).
Our experience after annotating the dataset is that the audio quality is, in many occasions, relatively mid-high.
To put this perception into context we make the following observation.
The notion of audio quality in datasets for sound recognition has been subject to changes over time, just as the notion of dataset size.
In the first editions of the DCASE Challenge, datasets recorded with professional equipment dominated, some of them being recorded with one single microphone/recorder model \cite{mesaros2017detection,Mesaros2016_EUSIPCO,Lafay2017,DCASE2017challenge}---this was the common quality standard at the time.
Then, AudioSet became popular, presenting an extreme diversity of audio qualities given its size.
In this case, a huge variety of devices and consumer electronics are used for recording YouTube \textit{videos} (where recording audio is not necessarily the main goal), and often including low SNR conditions, thus lowering the \textit{de facto} quality standard.
In our experience, after having used and listened to a portion of some of these datasets, and despite the diversity of Freesound, we speculate that the overall audio quality of FSD50K lies between the two aforementioned cases.


\subsubsection{Real-world Audio}
In many occasions, sound events in Freesound are real-world recordings of sound events happening in the wild, e.g., a car passing by.
However, it is not uncommon that some sound events are recorded under careful conditions in order to obtain clean and isolated high-quality sounds, as in a foley sound setting, e.g., the sound of tearing paper carefully located in front of a microphone.
Further, a few clips in Freesound consist of sound events purposefully generated with the sole objective of being recorded, e.g. a faked laughter. 
While these recordings are valuable for sound design, in some cases they could feature a lack of naturalness or acoustic mismatch with respect to sound events in the wild.
This may question the suitability of a portion of the data for learning sound recognizers to be deployed in the wild, where more adverse generation and recording conditions can be encountered.
To what extent this affects generalization of trained models to adverse scenarios is an open question. 
Mitigating this potential mismatch through robustness measures could be a research problem involving data augmentation \cite{salamon2017deep} and domain adaptation \cite{li2017large} techniques.


%============================================================================================
\subsection{Limitations}
\label{ssec:limit}
We believe highlighting the limitations of a dataset is important so that dataset users can take actions accordingly. The main limitations of FSD50K are as follows.

\subsubsection{Label Noise}
Throughout this paper we have mentioned the correctness and completeness of labels in different portions of the dataset.
While this was the goal, this is somewhat unrealistic as it would mean perfect accuracy of the candidate nomination system and of the human-provided labels.
In fact, as supervised learning research moves towards larger datasets, issues of label noise become inevitable.
For example, labeling error in AudioSet is estimated at above 50\% for $\approx$18\% of the classes.\textsuperscript{\ref{foot_aset_noise}} 
Similarly, ImageNet training data are often presumed to have correct labels, but it has been recently estimated that at least 100k images could be labeled incorrectly \cite{northcutt2019confident}.
In the SER field, label sets in not-small datasets are inherently noisy due to reasons such as sub-optimality of automatic methods used in the creation, or the difficulty of annotating audio---especially without visual cues and with large vocabularies.
Consequently, recent works have demonstrated the efficacy of label noise treatment 
in large datasets such as AudioSet \cite{fonseca2020addressing,kumar2019secost} and in mid-size datasets \cite{Fonseca2019learning,Fonseca2019model,iqbal2020learning}.
Despite our efforts to mitigate label noise in FSD50K, there are still a few concrete label noise issues.
While it is not common for dataset creators to explicitly highlight label noise problems in the proposed datasets \cite{gemmeke2017audio,deng2009imagenet}, next we identify the main sources of label noise in FSD50K, so that dataset users can leverage this information.

The main label noise problem in FSD50K is the existence of \textit{missing} “Present” labels (false negatives), that is, labels that would be included in an ideal, exhaustive annotation but which are missing from the current set.
Recent work identifies this as a pathology in AudioSet and proposes a method to tackle it \cite{fonseca2020addressing}.
This problem affects more the dev set due to the annotation process based on validation of nominated labels (Sec. \ref{ssec:task_val})---if sound events are not nominated by the system, they lack labels.
In our experience, this may happen with sound events that tend to be less represented by the Freesound user-provided tags, such as human or bird sounds when they are not the most relevant events in a clip.
Because the eval set received exhaustive annotation, this problem should be minimized as we get closer to a complete audio transcription.
Then, to a much lesser extent, two additional sources of missing labels exist.
First, the impossibility of propagating labels in the hierarchy when multiple ambiguous paths are encountered (Sec. \ref{ssec:postpro})---again, this affects more the dev set than the eval set, by dataset curation.
Second, some missing labels occur as the result of annotating with a finite vocabulary---there may be additional acoustic content \textit{out-of-vocabulary}.
Apart from missing labels, the other label noise problem that could be present is the existence of \textit{incorrect} “Present” labels (a false positive, and potentially a false negative if the true class exists \textit{in-vocabulary}).
This would be the result of human annotation errors despite the adoption of quality bootstrapping mechanisms such as training raters (sometimes using expert raters), using quality control checks when gathering annotations, or demanding inter-annotator agreement in most cases (sometimes between more than two raters).
Therefore, we expect incorrect labels to be rare.

Both missing and incorrect labels would be class-conditional (a.k.a. non-uniform noise \cite{arazo2019unsupervised}) as some classes are clearly more ambiguous than others, which affects both the nomination system and human labelling.
As mentioned, when labelling errors occur, the non-existent true labels can be either in-vocabulary or out-of-vocabulary, which pose different problems.
Further details about label noise characterization can be found in \cite{Fonseca2019learning}.
Being aware that label noise is unavoidable, users that detect labelling errors can report them via the companion site\textsuperscript{\ref{foot_companion}}.
In this way, amendments to be included in future versions of the dataset can be done collaboratively.

\subsubsection{Data Imbalance}
While some classes have abundant data, others are much less represented due to the data scarcity in Freesound and/or low performance of the nomination system.
Another source of imbalance is the variable length of clips---some classes tend to contain shorter/longer clips depending on the type of sound events and the preferences of Freesound users when recording them.
Finally, the hierarchical structure of the ontology favours data imbalance between classes in the different levels.

\subsubsection{Data Bias in Development Set}
Because we prioritized the eval set over the dev set, the development portion of a few classes is dominated by a few large uploaders.
Under the assumption that this signifies similar training examples in certain cases, this could create a data bias, which could be learnt by models \cite{lei2011user}.  
This happens mainly in a few instruments, e.g., \textit{Trumpet}, as some users upload many clips of the same class to Freesound.
Further analysis would be needed to determine if and how much this potential bias causes lack of generalization for these classes.

\subsubsection{Lack of Specificity in the Vocabulary}
Some leaf nodes in the ontology were merged to their parents due to data scarcity.
For instance, in the domestic sounds branch some leaf nodes (e.g. \textit{Blender}, \textit{Chopping (food)}, \textit{Toothbrush}) had to be merged with their parent \textit{Domestic sounds, home sounds}.
This motivated us to keep the latter as a valid class despite it being originally blacklisted in the ontology.
A natural extension of FSD50K is to grow some of these merged leaf nodes by adding more data.


%============================================================================================
\subsection{Applications}
\label{ssec:apps}
FSD50K allows evaluation of approaches for a variety of sound recognition tasks. 
The most evident is multilabel sound event classification with large vocabulary \cite{Fonseca2019audio}.
In this context, the proposed dataset supports several approaches such as learning sound event representations directly from waveforms \cite{cakir2016filterbank,park2020cnn}; analysis of label noise mitigation methods leveraging the non-exhaustive labeling of the dev set \cite{Fonseca2019learning,fonseca2020addressing,Fonseca2019model}; multimodal approaches using both audio and text information (e.g., using the provided Freesound tags) \cite{elizalde2019cross,favory2020coala}; evaluation of hierarchical classification via ontology-aware learning frameworks \cite{cramer2020chirping,shrivaslava2020mt,jati2019hierarchy}; or approaches specifically combining strong and weak labels \cite{kumar2017audio}.
By leveraging the common vocabulary between FSD50K and AudioSet, we hope that a number of tasks become possible, such as experimenting with domain adaptation techniques \cite{gharib2018unsupervised}, or cross-dataset evaluation \cite{bogdanov2016cross} under different acoustic conditions (see Sec. \ref{ssec:compare}).
Other tasks include but are not limited to: search result clustering in large vocabulary datasets \cite{favory2020search}, universal sound separation \cite{Kavalerov_WASPAA2019}, or active learning for sound event classification with large vocabulary. 
%Finally, the proposed eval set can be used as a benchmark beyond FSD50K.

In addition, the collection of these data has already accomplished several high-impact milestones for the research community.
The data curated has been used for a number of smaller datasets for sound event classification \cite{fonseca2018general,Fonseca2019learning,Fonseca2019audio} and source separation \cite{Wisdom_InPrep2020}, which add to previously existing datasets nourished from Freesound content \cite{salamon2014dataset,foster2015chime,piczak2015esc,stowell2013open,DCASE2017challenge}.
Likewise, from the beginning of its creation, FSD50K has enabled several sound recognition Challenges---specifically, DCASE 2018 Task 2 \cite{fonseca2018general}, DCASE 2019 Tasks 2 \cite{Fonseca2019audio} and 4 \cite{turpault2019sound}, and DCASE 2020 Task 4 \cite{turpault2020improving}.
We believe these multiple contributions demonstrate the value of this effort.


%============================================================================================
\subsection{FSD50K and AudioSet}
\label{ssec:compare}
We discuss the main similarities and differences between both datasets, some of them listed in Table~\ref{tab:fsd_aset}.
\begin{table}[ht]
%\vspace{-1mm}
\caption{Comparison of some properties of FSD50K and AudioSet.}
%\vspace{+3mm}
\centering
\begin{tabular}{lcc}
\toprule
             & \textbf{FSD50K} & \textbf{AudioSet} \\
\midrule
classes          & 200             & 527              \\
content          & waveform        & features        \\
%stability        & yes             & no             \\
dev clips        & 40,966          & $\approx$2M       \\
eval clips       & 10,231          & 20,383                  \\
%content license          & several CCs     & CC-BY-4.0        \\
clip length      & 0.3-30s       & $\approx$10s        \\
dev labeling      & CpI            & CpI             \\
eval labeling     & exhaustive     & CpI          \\
source          & Freesound audio  & Youtube video      \\
%\midrule
\bottomrule
\end{tabular}
\label{tab:fsd_aset}
%\vspace{-2mm}
\end{table}
Both datasets use the AudioSet Ontology for organization, however FSD50K uses a smaller subset.
All classes in FSD50K are represented in AudioSet, except \textit{Crash cymbal} as well as four classes that are blacklisted in AudioSet but not in FSD50K (\textit{Human group actions}, \textit{Human voice}, \textit{Respiratory sounds}, and \textit{Domestic sounds, home sounds}).
The reason to preserve these classes is that they aggregate clips from some of their children that were not considered large enough for the release.
FSD50K provides audio waveforms under several CC licenses as decided by Freesound users.
The official AudioSet release consists of audio features pre-computed at a time resolution of 960ms, released under CC-BY-4.0 license.
Apart from this, some AudioSet users attempt to download the corresponding video soundtracks from YouTube.
In terms of stability, FSD50K is released with permanent Digital Object Identifier downloadable as several zip files from its Zenodo page.\textsuperscript{\ref{foot_zenodo}}
AudioSet features can be downloaded as a tar.gz file from the AudioSet website.\footnote{\url{https://research.google.com/audioset/download.html}}
The original YouTube video soundtracks, however, are gradually disappearing as they are subject to deletions and other issues (see Sec. \ref{sec:intro}).
As seen in Table~\ref{tab:fsd_aset}, AudioSet's dev set is significantly larger than FSD50K's whereas AudioSet's eval set is roughly twice the FSD50K's eval set.
Since AudioSet has a vocabulary 2.6 times larger, this means that in a few classes there is more evaluation content in FSD50K than in AudioSet.
Clips in AudioSet last $\approx$10s, whereas in FSD50K their length varies from 0.3 to 30s.
As a consequence, label weakness is more homogeneous in AudioSet, whereas it varies significantly in FSD50K, sometimes yielding quasi-strong labels as clips get shorter, and sometimes yielding much weaker labels in the longest clips.
%This is especially beneficial for short events like door slams or snare drums.

In terms of labeling, FSD50K provides event predominance annotations while AudioSet only provides presence annotations.
While it is not easy to objectively compare both datasets in terms of label quality, we speculate that the labelling of both dev sets could be regarded as \textit{Correct but Potentially Incomplete} (CpI), i.e., both dev sets would be affected by a certain amount of missing labels. 
However, it seems reasonable to assume that, in the FSD50K portion of rather short sounds with PP annotations (see Sec. \ref{ssec:discussion}), the amount of missing labels is minimal.
The eval set of FSD50K was exhaustively annotated; therefore, absence of labels means absence of sound events (except human error).
By contrast, the eval annotations in AudioSet would be CpI.
Unlike AudioSet, FSD50K consistently provides all relevant labels in a hierarchical path, except in a few specific cases of ambiguous ancestors.
As additional resources, we provide the opportunity to flag labelling errors through the Freesound Annotator, additional metadata (Freesound tags for the audio clips as well as class-wise annotation FAQs), and open-source code for baseline experiments.

Finally, despite both datasets being highly heterogeneous, we make the following conjectures.
Audio clips in Freesound are typically recorded with the purpose of capturing audio, which is not necessarily the case in YouTube videos.
In addition, given the AudioSet size, its audio clips are presumably recorded with a higher diversity of devices.
As mentioned in Sec. \ref{ssec:discussion}, this would provide AudioSet with a higher diversity of audio qualities, often including more real-world and lower SNR conditions than Freesound audio.
In light of the above, a certain acoustic mismatch between both datasets may be expected.
In our view, both datasets suppose complementary resources for sound event research.
